Rethinking the Representation in Federated Unsupervised Learning with Non-IID Data

Federated learning achieves effective performance in modeling decentralized data. In practice, client data are not well-labeled, which makes it potential for federated unsupervised learning (FUSL) with non-IID data. However, the performance of existing FUSL methods suffers from insufficient representations, i.e., (1) representation collapse entanglement among local and global models, and (2) inconsistent representation spaces among local models. The former indicates that representation collapse in local model will subsequently impact the global model and other local models. The latter means that clients model data representation with inconsistent parameters due to the deficiency of supervision signals. In this work, we propose FedU2 which enhances generating uniform and unified representation in FUSL with non-IID data. Specifically, FedU2 consists of flexible uniform regularizer (FUR) and efficient unified aggregator (EUA). FUR in each client avoids representation collapse via dispersing samples uniformly, and EUA in server promotes unified representation by constraining consistent client model updating. To extensively validate the performance of FedU2, we conduct both cross-device and cross-silo evaluation experiments on two benchmark datasets, i.e., CIFAR10 and CIFAR100.

==> chapters/draft.tex <==
 \section{Introduction}
%  \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figs/motivation.png} 
% \caption{Motivation of \modelname.}
% \label{fig:motivation}
% \end{figure}

To resolve cross-silo and privacy regularization,
Federated learning (FL)~\cite{FedAvg} is boosting to model decentralized data in both academia and industry.
% 
Because FL collaborates client models trained on decentralized data, and seeks to a performant global model without transferring data.
% 
% However, most of the existing work focuses on improving performance, communication cost, and convergences in FL with non-IID data, with the assumption that clients contain labels to capture supervised signals. 
% % 
However, conventional FL work mostly assumes that client data is well-labeled, which is less practical in real-world applications.
% 
In this work, we consider federated unsupervised learning (\problem) with non-IID data~\cite{fuslSurveyFengda,fuslSurveyYangQiang}, i.e., modeling unified representation among imbalanced, unlabeled, and decentralized client data.
% modeling imbalanced decentralized client data without access to data labels.

% 
% 1. 直接将centralized USL 用于FL的limitations
% 2. 现有USL FL 方法的不足
% 2.1 pseudo label-> computation
% 2.2 FedCA-> privacy
% 2.3 self-supervised: overlook the i-i consistency & i-c consistency
% orchestra consider i-c consistency, but requires heavy computation on clustering, and may suffer  from randomness
% 
Existing \problem~methods can be grouped into three categories: (1) collaborates existing centralized unsupervised learning model with FL framework, (2) measures client divergence with data sharing,
 and (3) applies self-supervised learning for \problem.
% 
The first category 
cannot obtain satisfying results, because it fails to capture the divergence among clients~\cite{fedu}.
% 
The second category requires an external dataset to alleviate client inconsistency~\cite{zhang2020federated} or clustering clients based on decentralized data~\cite{wu2021federated}, which leaks privacy inevitably.
% 
The third category utilizes self-supervised model and aggregate models with divergence-aware updating, e.g., \cite{fedu,fedema}, knowledge distillation, e.g.,~\cite{fedx}, or tracking a set of global centroids by local-global clustering~\cite{orchestra}, improving the performance of \problem~with non-IID data without sharing data.

% 
Though the current third category captures the inconsistency among clients well, the performance of \problem~is still hindered due to two challenges.
% 
\textit{CH1: Mitigating representation collapse, i.e., dimensional collapse~\cite{} and complete collapse\cite{}},
% so as to obtain diverse representations inherent class-imbalanced client data},
and \textit{CH2: Obtaining consistent representations space among heterogeneous clients}.
% 
The former indicates that existing \problem~methods overlook the representation collapse brought by modeling real-world application client data, i.e., data follows class-imbalanced, even long-tailed distribution~\cite{imbalancedssl}.
% 
FedDecorr~\cite{feddecorr} is the first to discover and tackle dimensional collapse in federated learning, i.e., 
local client dimensional collapse deteriorates the global representation.
% 
However, FedDecorr simply decorrelates dimensional-wise representation space in federated supervised learning via analyzing the gradient dynamics of cross-entropy loss.
% 
With the reliability of label signal, FedDecorr fails to alleviate both dimensional collapse and complete collapse simultaneously.
% 
Though representation collaspse is widely studied in centralized self-supervised space using (1) contrastive learning, (2) asymmetric architecture modeling~\cite{byol}, and (3) feature decorrelation~\cite{btloss}. 
% 
Directly pretraining unlabeled client data via existing centralized self-supervised learning, prevent its capability to generalize unified representations.
% 
Because these methods typically are either explicit or implicit k-Means that suffers from degeneration solutions~\cite{pretrain_longtail}. 

The latter challenge refers to optimize inconsistent client model parameters toward inconsistent parameter space, bringing indistinguishable representations on global model.
% 
Most of the existing \problem~methods aggregate activate client model with the ratio of samples, i.e., FedAvg~\cite{FedAvg}, which fails to tackle the client shift from global optimum to local optimum and brings sub-optimal results~\cite{fedprox,ldawa}.
% 
To mitigate this, FedEMA~\cite{fedema} and FedU~\cite{fedu} restrict the extreme divergent client from aggregating with a fixed or adaptive threshold.
% 
limitation 1
% 
Orchestra~\cite{orchestra} derives from K-Fed~\cite{kfed} to search consistent global supervision signal, via clustering local cluster proxy in server.
% 
This brings additional computation cost and memory cost for clustering and sample representation bank.
% 
Recently, L-DAWA~\cite{ldawa} corrects the \problem~optimization trajectory by measuring and scaling angular divergence among client model in a layer-wise way.
% 
However, this kind of method bring extra computation cost.





Firstly, current self-supervised methods \textit{fail to sufficiently represent the minority of imbalanced data} (\textbf{CH 1}).
% 
As depicted in Fig.~\ref{fig:motivation} (a), during modeling the imbalanced data locally, the model updating accounts more for the majority of data samples, which represents the minority of data insufficiently and inaccurately.
% 
Secondly, \problem~\textit{faces the intra-client inconsistency and the inter-client inconsistency simultaneously} (\textbf{CH 2}), both of which prevent capturing deterministic clustering signals.
% 
In Fig.~\ref{fig:motivation}, client 2 suffers from instance-instance inconsistency, which brings an incorrect decision boundary between the green circles and green stars.
% 
In the client of \problem, each model is unaware of the whole data distribution, failing to similarly represent two samples among different clients but the same cluster.
% Instance-instance consistency focuses on getting tighter clustering, however, it fails to infer the distance between two samples among different clients but the same cluster.
% % 
% The instance-cluster consistency will encourage the consistent ground truth among decentralized data, while, it cannot be reliable on random clustering.
% 
\cite{orchestra} considers the instance-cluster consistency and \cite{fedssl} maintains the instance-instance consistency, however, neither of them tackles both of the consistencies at the same time.
% 
Lastly, clustering global centroids to mitigate client divergence in \problem~
\textit{is sensitive to randomness} (\textbf{CH 3}), i.e., randomly initialized high-dimensional feature representations can be assigned differently.
% 
Besides, computing in high-dimensional space requires quite a large time complexity, which calls for a quick converge and robust clustering methods for \problem.
% 



To fill this gap, we propose \modelname, which consists of 
three key components that tackle the above limitations, respectively.
% 
For tackling \textbf{CH 1}, we devise neighbor augmentation module to enhance the sample representation with its neighbor, i.e., samples with high similarity.
% 
We first compute the similarity among a batch of data samples, find the neighbors of data samples based on the similarity, and then enhance the data feature representation based on attentive graph augmentation.
% 
Aiming at \textbf{CH 2}, we optimize toward contrastive discrimination and cross-supervision objectives simultaneously, to maintain the intra- and inter-cluster relations in decentralized data.
% 
We capture the instance-instance contrastive discrimination, which encourages model to represent data samples of the sample cluster similarly, and push the data samples of different clusters away.
% 
We maintain the instance-cluster cross-supervision, i.e., sharing a set of global centroids among clients, to keep the representation of the same cluster consistent, among clients.
% 
To mitigate \textbf{CH 3}, we devise cascade Bregman power K-means federated clustering to obtain clustering centroids insensitive to randomness and efficient in high-dimensional computation.
% 
We measure the data dissimilarity based on the Bregman divergence and optimize for Power K-means, which first constructs a set of data proxy locally, and establish global centroids based on proxies in server.
% 

In the summary, we are the first, as far as we know, to enhance \problem~with non-IID data using graph augmentation.
% 
\xenia{todo}
The main contributions are :
(1)
We adopt uniformly distributed and fixed class prototypes in hyperbolic space to alleviate the performance degradation caused by the class statistics shifting. 
%
(2)
We present the first attempt to sufficiently leverage hyperbolic representation space to capture hierarchical information in low-dimensional space for FL.
% 
(3) We optimize the combination of different client deviations to a Pareto stationary point, which minimizes the impact of the inconsistent updating clients in federated aggregation.
%
(4) Extensive experiments conducted on four benchmark datasets prove the effectiveness of \modelname~and its modules, 
compared with the state-of-the-art FL methods.






$13 \mathrm{UOT} / \mathrm{PUOT}$ on $\ell_2$-Norm Constraints
Then we introduce UOT with $\ell_2$-norm.
$$
\begin{aligned}
\min _{\pi_{i, j} \geq 0} J & =\operatorname{vec}(\boldsymbol{C})^{\top} \operatorname{vec}(\boldsymbol{\pi})+\frac{\tau_a}{2}\left\|\boldsymbol{\Phi}_{\mathrm{r}} \operatorname{vec}(\boldsymbol{\pi})-\boldsymbol{a}\right\|_2^2+\frac{\tau_b}{2}\left\|\boldsymbol{\Phi}_{\mathrm{c}} \operatorname{vec}(\boldsymbol{\pi})-\boldsymbol{b}\right\|_2^2 \\
& =\operatorname{vec}(\boldsymbol{C})^{\top} \operatorname{vec}(\boldsymbol{\pi})+\frac{\tau_a}{2}\left(\boldsymbol{\Phi}_{\mathrm{r}} \operatorname{vec}(\boldsymbol{\pi})-\boldsymbol{a}\right)^{\top}\left(\boldsymbol{\Phi}_{\mathrm{r}} \operatorname{vec}(\boldsymbol{\pi})-\boldsymbol{a}\right)+\frac{\tau_b}{2}\left(\boldsymbol{\Phi}_{\mathrm{c}} \operatorname{vec}(\boldsymbol{\pi})-\boldsymbol{b}\right)^{\top}\left(\boldsymbol{\Phi}_{\mathrm{c}} \operatorname{vec}(\boldsymbol{\pi})-\boldsymbol{b}\right) \\
& =\operatorname{vec}(\boldsymbol{C})^{\top} \operatorname{vec}(\boldsymbol{\pi})+\frac{\tau_a}{2} \operatorname{vec}(\boldsymbol{\pi})^{\top} \boldsymbol{\Phi}_{\mathrm{r}}^{\top} \boldsymbol{\Phi}_{\mathrm{r}} \operatorname{vec}(\boldsymbol{\pi})+\frac{\tau_b}{2} \operatorname{vec}(\boldsymbol{\pi})^{\top} \boldsymbol{\Phi}_{\mathrm{c}}^{\top} \boldsymbol{\Phi}_{\mathrm{c}} \operatorname{vec}(\boldsymbol{\pi})-\tau_a \boldsymbol{a}^{\top} \boldsymbol{\Phi}_{\mathrm{r}} \operatorname{vec}(\boldsymbol{\pi})-\tau_b \boldsymbol{b}^{\top} \boldsymbol{\Phi}_{\mathrm{c}} \operatorname{vec}(\boldsymbol{\pi})+\cdots \\
& =\frac{1}{2} \operatorname{vec}(\boldsymbol{\pi})^{\top}\left(\tau_a \boldsymbol{\Phi}_{\mathrm{r}}^{\top} \boldsymbol{\Phi}_{\mathrm{r}}+\tau_b \boldsymbol{\Phi}_{\mathrm{c}}^{\top} \boldsymbol{\Phi}_{\mathrm{c}}\right) \operatorname{vec}(\boldsymbol{\pi})+\left(\operatorname{vec}(\boldsymbol{C})-\tau_a \boldsymbol{\Phi}_{\mathrm{r}}^{\top} \boldsymbol{a}-\tau_b \boldsymbol{\Phi}_{\mathrm{c}}^{\top} \boldsymbol{b}\right)^{\top} \operatorname{vec}(\boldsymbol{\pi})+\cdots
\end{aligned}
$$
The constraints are defined as:
Meanwhile we can denote that:
$$
\begin{array}{r}
\tau_a \boldsymbol{\Phi}_{\mathrm{p}}^{\top} \boldsymbol{\Phi}_{\mathrm{r}}+\tau_b \boldsymbol{\Phi}_c^{\top} \boldsymbol{\Phi}_c=\boldsymbol{Q} \\
\operatorname{vec}(\boldsymbol{C})-\tau_a \boldsymbol{\Phi}_{\mathrm{r}}^{\top} \boldsymbol{a}-\tau_b \boldsymbol{\Phi}_c^{\top} b=\boldsymbol{w}
\end{array}
$$
Then we can optimize $\pi$ as:
$$
\operatorname{vec}\left(\pi^{(\text {new })}\right)=\max \left(0, \operatorname{vec}\left(\pi^{\text {(old })}\right)-\eta^* \frac{\partial J}{\partial \operatorname{vec}\left(\pi^{(\text {old })}\right)}\right) \quad \text { and } \quad \eta^*=\frac{\left(\boldsymbol{Q}_{\operatorname{vec}}\left(\pi^{(\text {old })}\right)+\boldsymbol{w}\right)^{\top}\left(\boldsymbol{Q}_{\operatorname{vec}}\left(\boldsymbol{\pi}^{(\text {old })}\right)+\boldsymbol{w}\right)}{\left(\boldsymbol{Q}_{\operatorname{vec}}\left(\boldsymbol{\pi}^{(\text {old })}\right)+\boldsymbol{w}\right)^{\top} \boldsymbol{Q}\left(\boldsymbol{Q} \operatorname{vec}\left(\boldsymbol{\pi}^{(\text {old })}\right)+\boldsymbol{w}\right)}
$$
Hence we can optimize the optimize the results on $\pi$.




\xenia{below is copied from FAMO}

3.1 Balanced Rate of Loss Improvement
At time $t$, define the rate of improvement for task $i$ as
$$
c^i\left(\alpha, d_t\right)=\frac{L^i\left(\theta_t\right)-L^i\left(\theta_t-\alpha d_t\right)}{\Delta_t^i}, \text { where } \Delta_t^i=L^i\left(\theta_t\right)+\epsilon
$$
Here, $\epsilon \in \mathbb{R}^{+}$is a small constant that prevents division by zero. FAMO then seeks an update $d_t$ that encourages a larger worst-case rate of improvement across all tasks $\left(\frac{1}{2}\left\|d_t\right\|\right.$ is subtracted to prevent an under-specified optimization problem where the objective can be infinitely large):
$$
\max _{d_t \in \mathbb{R}^m} \min _{i \in[K]} \frac{1}{\alpha} c^i\left(\alpha, d_t\right)-\frac{1}{2}\left\|d_t\right\|^2 .
$$
3
When the step size $\alpha$ is small, (5) transforms into
$$
\max _{d_t \in \mathbb{R}^m} \min _{i \in[K]} \frac{\nabla L^i\left(\theta_t\right)^{\top} d_t}{\Delta_t^i}-\frac{1}{2}\left\|d_t\right\|^2=\left(\nabla \log \Delta_t^i\right)^{\top} d_t-\frac{1}{2}\left\|d_t\right\|^2 .
$$
Now, we have the following proposition to ensure that the solution to (6) results in equal rate of improvement across all task losses.

Proposition 3.1. Assume $\left\{L^i\right\}$ are smooth, denote $d^*$ as the maximizer of (6). Then $\forall i \neq j \in[K]$,
$$
\lim _{\alpha \rightarrow 0} \frac{L^i\left(\theta_t\right)-L^i\left(\theta_t-\alpha d^*\right)}{\Delta_t^i}=\lim _{\alpha \rightarrow 0} \frac{L^j\left(\theta_t\right)-L^j\left(\theta_t-\alpha d^*\right)}{\Delta_t^j} .
$$
The proof of Proposition 3.1 is in Appendix E. Instead of solving the primal problem in (6) where $d \in \mathbb{R}^m$ ( $m$ can be the size of a neural network), we consider its dual problem in the following.
Proposition 3.2. Denote $\Delta_t=\left(\Delta_t^1, \ldots, \Delta_t^K\right)^{\top}$. The dual form for (6) is
$$
\min _{\boldsymbol{z} \in \mathbb{S}^K} \frac{1}{2}\left\|\left(\nabla \log \boldsymbol{\Delta}_t\right) \boldsymbol{z}\right\|^2 .
$$
Here, $z \in \mathbb{S}^K$ is the dual decision variable and can be viewed as the weighting of task losses. The duality gap is zero as the primal objective is maximizing an objective that is concave in $d$. Therefore, (7) provides a natural objective for optimizing the task weights $\boldsymbol{z}$ for balancing task losses. Because optimizing $\left(\log \boldsymbol{\Delta}_t\right)^{\top} \boldsymbol{z}^*$, where $\boldsymbol{z}^*$ is the solution to (7), will result in equal rate descent. Note that (7) can be viewed as applying MGDA $[9,34]$ to the log of all task losses (See Appendix A).
3.2 Fast Approximation
Instead of fully solving (7) at each optimization step, FAMO performs a single-step gradient descent on $\boldsymbol{z}$, which amortizes the computation over the optimization trajectory:
$$
\boldsymbol{z}_{t+1} \leftarrow \boldsymbol{z}_t-\tilde{\beta} \tilde{\delta}, \quad \text { where } \tilde{\delta}=\nabla_{\boldsymbol{z}}\left(\frac{1}{2}\left\|\left(\nabla \log \boldsymbol{\Delta}_t\right)^{\top} \boldsymbol{z}\right\|^2\right)=\left(\nabla \log \boldsymbol{\Delta}_t\right)^{\top}\left(\nabla \log \boldsymbol{\Delta}_t\right) \boldsymbol{z}_t .
$$
But then, assume $\theta_{t+1} \leftarrow \theta_t-\eta \nabla \log \left(\boldsymbol{\Delta}_t\right) \boldsymbol{z}$, one can approximate (8) by:
$$
\left(\nabla \log \boldsymbol{\Delta}_t\right)^{\top}\left(\nabla \log \boldsymbol{\Delta}_t\right) \boldsymbol{z}_t \approx \frac{1}{\eta}\left(\log \boldsymbol{\Delta}_t-\log \boldsymbol{\Delta}_{t+1}\right) .
$$
In practice, it is hard to guarantee that after performing the update on $\boldsymbol{z}$, it still remains in $\mathbb{S}_K$. Therefore, we do a re-parameterization and let $\boldsymbol{z}_t=\operatorname{Softmax}\left(\boldsymbol{w}_t\right)$, where $\boldsymbol{w}_t \in \mathbb{R}^K$ is the softmax logits and is unconstrained. Consequently, we have the following approximate update on $\boldsymbol{w}$ from (8):
$$
\boldsymbol{w}_{t+1} \leftarrow \boldsymbol{w}_t-\beta \delta, \quad \text { where } \delta=\left(\begin{array}{c}
\nabla^{\top} z^1(\boldsymbol{w}) \\
\vdots \\
\nabla^{\top} z^K(\boldsymbol{w})
\end{array}\right)^{\top}\left(\log \boldsymbol{\Delta}_t-\log \boldsymbol{\Delta}_{t+1}\right) .
$$
Remark: While in principle, it is possible to perform gradient descent on $\boldsymbol{z}$ for other gradient manipulation methods, we will demonstrate in Appendix B that not all such updates can be easily approximated using the change in losses.

3.3 Practical Implementation
To facilitate practical implementation, we present two modifications to the update in (10).
1. Re-normalization: Assume we follow the update $\theta_{t+1} \leftarrow \theta_t-\eta \nabla \log \left(\boldsymbol{\Delta}_t\right) \boldsymbol{z}$, then when $\Delta_t^i$ is small, one observes that $\nabla \log \left(\Delta_t^i\right) v^i=\nabla L^i\left(\theta_t\right) v^i / \Delta_t^i$ can be large, consequently causing $\|d\|=\left\|\nabla \log \Delta_t \boldsymbol{z}_t\right\|$ to be large as well. To mitigate this problem, we re-normalize the task weighting back into the probability simplex by dividing a constant $c_t$ per step:
$$
\theta_{t+1} \leftarrow \theta_t-\alpha\left(\nabla \log \boldsymbol{\Delta}_t\right) \frac{\boldsymbol{z}_t}{c_t}, \text { where } c_t=\left(\boldsymbol{z}_t \oslash \boldsymbol{\Delta}_t\right)^{\top} \mathbf{1}
$$
Here, $\oslash$ denotes element-wise division. By doing so, (11) is equivalent to
$$
\theta_{t+1} \leftarrow \theta_t-\alpha \nabla \boldsymbol{L}\left(\theta_t\right) \boldsymbol{v}_t, \text { where } \boldsymbol{v}_t=\frac{\boldsymbol{z}_t}{c_t} \oslash \boldsymbol{\Delta}_t \in \mathbb{S}^K .
$$
4
2. Regularization: Ideally, one would want to fully optimize (7) at each step $t$. But in (10) we amortize the update over time. But as the loss objectives $\boldsymbol{L}$ are also changing dynamically, it makes sense to focus more on the recent updates of $\boldsymbol{w}$ [45]. To this end, we introduce an $\ell_2$ regularization term that decays the past updates on $w$ :
$$
\boldsymbol{w}_t \leftarrow \boldsymbol{w}_{t-1}-\beta\left(\delta+\gamma \boldsymbol{w}_{t-1}\right) .
$$
Here $\gamma \in \mathbb{R}^{+}$is a hyperparameter that controls the decay rate and hence $\|\boldsymbol{w}\|$.
We provide the complete FAMO algorithm in Algorithm 1 and its pseudocode in Appendix C.
3.4 Stationary Points of FAMO
One way to characterize FAMO's behavior is to understand the stationary points of the continuoustime limit of FAMO (i.e. when step sizes $(\alpha, \beta)$ shrink to zero). From Algorithm 1, one can derive the following non-autonomous dynamical system (assuming $\left\{L^i\right\}$ are all smooth):
$$
\left\{\begin{array}{l}
\frac{d}{d t} \theta_t=-\left(\nabla \log \boldsymbol{\Delta}_t\right) \operatorname{Softmax}\left(\boldsymbol{w}_t\right) \\
\frac{d}{d t} \boldsymbol{w}_t=A_t\left(\frac{d}{d t} \log \boldsymbol{\Delta}_t\right)-\gamma \boldsymbol{w}_t
\end{array} \quad \text { where } \quad A_t=\left(\begin{array}{c}
\nabla^{\top} z^1(\boldsymbol{w}) \\
\vdots \\
\nabla^{\top} z^K(\boldsymbol{w})
\end{array}\right) .\right.
$$
When the dynamical system (14) reaches its stationary points (or fixed points):
$$
\left\{\begin{array} { l l } 
{ \frac { d } { d t } \theta } & { = 0 } \\
{ \frac { d } { d t } \boldsymbol { w } } & { = \mathbf { 0 } }
\end{array} \stackrel { ( a ) } { \Longrightarrow } \left\{\begin{array} { l l } 
{ \frac { d } { d t } \boldsymbol { \Delta } } & { = \mathbf { 0 } } \\
{ ( \nabla \operatorname { l o g } \boldsymbol { \Delta } ) \operatorname { S o f t m a x } ( \boldsymbol { w } ) } & { = \mathbf { 0 } }
\end{array} \stackrel { ( b ) } { \Longrightarrow } \left\{\begin{array}{ll}
\boldsymbol{w} & =\mathbf{0} \\
\nabla\left(\log \boldsymbol{\Delta}^{\top} \mathbf{1}\right) & =0 .
\end{array}\right.\right.\right.
$$
Here, $(a)$ is straightforward as $\frac{d}{d t} \theta=0$. (b) is because when $\frac{d}{d t} \boldsymbol{\Delta}=0$ and $\frac{d}{d t} \boldsymbol{w}=0$, since $\gamma>0$, the second term in (14) indicates that $\boldsymbol{w}=0 \Longrightarrow \operatorname{Softmax}(\boldsymbol{w}) \stackrel{d t}{=}(1 / K, \ldots, 1 / K)^{\top}$. As a result, with $\frac{d}{d t} \theta=0$, we have $(\nabla \log \boldsymbol{\Delta})(1 / K, \ldots, 1 / K)^{\top}=\nabla\left(\log \boldsymbol{\Delta}^{\top} \mathbf{1}\right)=0$. Therefore, the minimum points of $\sum_{k=1}^K \log \left(L^i(\theta)+\epsilon\right)$ are all stationary points of (14).


Gaussian distribution
Now consider the case where we have a known mean $\mu$ and variance $\sigma^2$. We will consider $x \in(-\infty, \infty)$. Because variance is the expectation of the squared deviation of a random variable $x$ from its mean, it suffices to introduce the constraint
$$
\int_{-\infty}^{\infty}(x-\mu)^2 p(x) d x=\sigma^2
$$
which we will consider along with normalization when maximizing the entropy.
This leads to the Lagrangian
$$
J\left(p(x), \lambda_0, \lambda_1\right)=-\int_{-\infty}^{\infty} p(x) \ln p(x) d x+\lambda_0\left(\int_{-\infty}^{\infty} p(x) d x-1\right)+\lambda_1\left(\int_{-\infty}^{\infty}(x-\mu)^2 p(x) d x-\sigma^2\right)
$$
which, when differentiated with respect to $p(x)$ and set equal to zero, yields
$$
\frac{\partial J\left(p(x), \lambda_0, \lambda_1\right)}{\partial p(x)}=-\ln p(x)-1+\lambda_0+\lambda_1(x-\mu)^2=0
$$
which gives us an expression for $p(x)$ as
$$
p(x)=\exp \left(\lambda_0-1\right) \exp \left(\lambda_1(x-\mu)^2\right)
$$

For the first constraint, we find that
$$
\begin{aligned}
\int_{-\infty}^{\infty} p(x) d x & =1 \\
\int_{-\infty}^{\infty} \exp \left(\lambda_0-1\right) \exp \left(\lambda_1(x-\mu)^2\right) d x & =1 \\
\exp \left(\lambda_0-1\right) \int_{-\infty}^{\infty} \exp \left(\lambda_1(x-\mu)^2\right) d x & =1 \\
\exp \left(\lambda_0-1\right) \sqrt{\frac{\pi}{-\lambda_1}} & =1 \\
\exp \left(\lambda_0-1\right) & =\sqrt{\frac{-\lambda_1}{\pi} .}
\end{aligned}
$$

And for the second constraint we find
$$
\begin{aligned}
\int_{-\infty}^{\infty}(x-\mu)^2 p(x) d x & =\sigma^2 \\
\int_{-\infty}^{\infty} \sqrt{\frac{-\lambda_1}{\pi}}(x-\mu)^2 \exp \left(\lambda_1(x-\mu)^2\right) d x & =\sigma^2 \\
\sqrt{\frac{-\lambda_1}{\pi}} \int_{-\infty}^{\infty}(x-\mu)^2 \exp \left(\lambda_1(x-\mu)^2\right) d x & =\sigma^2 \\
\sqrt{\frac{-\lambda_1}{\pi}} \cdot \frac{1}{2} \sqrt{\frac{\pi}{-\lambda_1^3}} & =\sigma^2 \\
\lambda_1 & =-\frac{1}{2 \sigma^2} .
\end{aligned}
$$

Which allows us to say that
$$
\exp \left(\lambda_0-1\right)=\frac{1}{\sqrt{2 \pi \sigma^2}}
$$

Putting this all together yields the Gaussian, or normal distribution
$$
p(x)=\frac{1}{\sqrt{2 \pi \sigma^2}} \exp \left(-\frac{(x-\mu)^2}{2 \sigma^2}\right)
$$




Specifically, we first define the contribution of each client for aggregating a global model, and seek a direction that deviates from the smallest overall client contribution as much as possible.
% 
To avoid the overwhelming computation cost, we then convert
% Specifically, we avoid computing all task gradients by constraining an approximately similar optimization among all clients.
% % 
% Therefore, we can achieve an aggregation with Pareto optimal performance, benefiting ...
% In details, we rewrite Eq.~\eqref{eq:fusl_problem} in the form of deviations, i.e.,
% \begin{equation}
% \label{eq:agg_grad}
%     \Delta_{\boldsymbol{\theta}}^{t+1} = \Sigma_{k=1}^K p_k \Delta_{\boldsymbol{\theta}_{k}}^{t+1},
% \end{equation}
% where $\boldsymbol{\theta}^{t}_g$ is the global model, $\boldsymbol{\theta}_k^{t}$ is the local model of the client $k$ at $t-$th communication, $\Delta_{\boldsymbol{\theta}_g}^{t+1}=\boldsymbol{\theta}_g^{t+1} - \boldsymbol{\theta}_g^{t}$ and $\Delta_{\boldsymbol{\theta}_{k}}^{t+1}=\boldsymbol{\theta}_k^{t+1}-\boldsymbol{\theta}_g^{t}$.\xenia{rethink}
% %
% 
In a greedy way, we encourage global model to update towards a direction that corrects more for the aggregation with the smallest clients' contribution rate:
\begin{equation}
\max _{\boldsymbol{d}^t \in \mathbb{R}^{K\times m}} \min _{\boldsymbol{p} \in \mathbb{S}^K} \frac{1}{\eta} \sum_{k=1}^{K} p_k c_k(\eta, \boldsymbol{d}^t)-\frac{1}{2}\left\|\boldsymbol{d}^t\right\|^2 ,
\end{equation}
where the extra $-\frac{1}{2} \|\boldsymbol{d}\|^2$ prevents infinitely large objectives, and $\mathbb{S}^K=\{\boldsymbol{p}\in \mathbb{R}^K | \boldsymbol{p}^\top \boldsymbol{1}=1\}$.
% 
Assuming step size $\eta$ is small,
the global model updating can be approximated as $u_k\left(\boldsymbol{\theta}^{t}_g\right)-u_k\left(\boldsymbol{\theta}^{t+1}_g\right) \approx \eta \nabla\tilde{u}_k(\boldsymbol{\theta}^{t}_g)\boldsymbol{d}^t$,
we can further obtain:
\begin{equation}
\small
\begin{aligned}
\max _{\boldsymbol{d}^t \in \mathbb{R}^{K\times d}} \min _{\boldsymbol{p} \in \mathbb{S}^K} {(\Sigma_{k=1}^{K} p_k\nabla\log \tilde{u}_k \left(\boldsymbol{\theta}^{t}\right))}^\top \boldsymbol{d}^t - \frac{1}{2}\|\boldsymbol{d}^t\|^2\\
=  \min _{\boldsymbol{p} \in \mathbb{S}^K} \max _{\boldsymbol{d}^t \in \mathbb{R}^{K\times d}} {((\nabla\log \tilde{\boldsymbol{u}}^t)}\boldsymbol{p} )^\top\boldsymbol{d}^t - \frac{1}{2}\|\boldsymbol{d}^t\|^2
\end{aligned}
\label{eq:famo_obj}
\end{equation}
% 
The optimal updating direction can be reached when $(\nabla\log \tilde{\boldsymbol{u}})\boldsymbol{p}^* =\boldsymbol{d}^*$ where $\tilde{\boldsymbol{u}}= (\tilde{u}_1,\dots,\tilde{u}_K )$, and $\tilde{u}_k$ is short for $\tilde{u}_k(\boldsymbol{\theta})$.
% % 
Since the inner of Eq.\eqref{eq:famo_obj} is linear, we can change the min and max, then obtain a strong dual form that reduces the computation overhead with dual variable $\boldsymbol{p}$:
\begin{equation}
\boldsymbol{J} =\min _{\boldsymbol{p}\in \mathbb{S}^K} \frac{1}{2} \|{(\nabla\log \tilde{\boldsymbol{u}}^t)}\top \boldsymbol{p}\|^2.
\label{eq:famo_dual}
\end{equation}

% 
Hence, we can optimize in a regularization, i.e.,
% 
\begin{equation}
\small
\boldsymbol{w}^{t+1} \leftarrow \boldsymbol{w}^t-\beta \left(\delta + \gamma \boldsymbol{w}^t\right), 
\end{equation}
where $\delta=\nabla_{z} \boldsymbol{J} \nabla_{w} z(\boldsymbol{w})
=\left(\nabla^{\top} z^1(\boldsymbol{w}), \dots, \nabla^{\top} z^K(\boldsymbol{w})\right)\left(\log \tilde{\boldsymbol{u}}^t-\log \tilde{\boldsymbol{u}}^{t+1}\right)$, and we assume to approximate gradient via $\nabla_{z} \boldsymbol{J}= \left(\nabla \log \tilde{\boldsymbol{u}}^t\right)^{\top}\left(\nabla \log \tilde{\boldsymbol{u}}^t\right) \boldsymbol{z}^t \approx \frac{1}{\eta}\left(\log \tilde{\boldsymbol{u}}^t-\log \tilde{\boldsymbol{u}}^{t+1}\right).$
% 
To avoid large uncontrollable update direction, we normalize the task weights by dividing a constant per step:
% and further regularize the decay rate:
\begin{equation}
\boldsymbol{\theta}^{t+1} \leftarrow \boldsymbol{\theta}^t-\eta \left(\nabla \log \tilde{\boldsymbol{u}}^t\right) \frac{\boldsymbol{z}_t}{c_t},
\end{equation}
 where $c_t=\left(\boldsymbol{z}_t \oslash \tilde{\boldsymbol{u}}^t\right)^{\top} \mathbf{1}$.

\begin{theorem}[Stationary Points for \moduleB]
The minimum points of $\Sigma^K_{k=1}\log(\tilde{u}_k)$ are all stationary points for the non-autonomous dynamical system of \moduleB~as below:
\begin{equation}
\left\{\begin{array}{l}
\small
\frac{d}{d t} \boldsymbol{\theta}^t=-\left(\nabla \log \tilde{\boldsymbol{u}}^t\right) \operatorname{Softmax}\left(\boldsymbol{w}^t\right) \\
\frac{d}{d t} \boldsymbol{w}^t=A^t\left(\frac{d}{d t} \log \tilde{\boldsymbol{u}}^t\right)-\gamma \boldsymbol{w}^t
\end{array}\right.
\end{equation}
where $A^t={\left(\nabla^{\top} p_1(\boldsymbol{w}), \dots,\nabla^{\top} p_K(\boldsymbol{w})\right)}^\top $.
\end{theorem}




Then we define the multi-objective optimization of client contribution rate
% 
% In a greedy way, we encourage global model to update towards a direction that corrects more for the aggregation with the smallest overall contribution rate
:
\begin{equation}
\max _{\boldsymbol{d}^t \in \mathbb{R}^{K\times m}} \min _{\boldsymbol{p} \in \mathbb{S}^K} \frac{1}{\eta} \sum_{k=1}^{K} p_k c_k(\eta, \boldsymbol{d}^t)-\frac{1}{2}\left\|\boldsymbol{d}^t\right\|^2 ,
\end{equation}
where the extra $-\frac{1}{2} \|\boldsymbol{d}\|^2$ prevents infinitely large objectives, and $\mathbb{S}^K=\{\boldsymbol{p}\in \mathbb{R}^K | \boldsymbol{p}^\top \boldsymbol{1}=1\}$.
% 
Assuming step size $\eta$ is small,
the global model updating can be approximated as $u_k\left(\boldsymbol{\theta}^{t}_g\right)-u_k\left(\boldsymbol{\theta}^{t+1}_g\right) \approx \eta \nabla\tilde{u}_k(\boldsymbol{\theta}^{t}_g)\boldsymbol{d}^t$,
we can further obtain:
\begin{equation}
\small
\begin{aligned}
\max _{\boldsymbol{d}^t \in \mathbb{R}^{K\times d}} \min _{\boldsymbol{p} \in \mathbb{S}^K} {(\Sigma_{k=1}^{K} p_k\nabla\log \tilde{u}_k \left(\boldsymbol{\theta}^{t}\right))}^\top \boldsymbol{d}^t - \frac{1}{2}\|\boldsymbol{d}^t\|^2\\
=  \min _{\boldsymbol{p} \in \mathbb{S}^K} \max _{\boldsymbol{d}^t \in \mathbb{R}^{K\times d}} {((\nabla\log \tilde{\boldsymbol{u}}^t)}\boldsymbol{p} )^\top\boldsymbol{d}^t - \frac{1}{2}\|\boldsymbol{d}^t\|^2,
\end{aligned}
\label{eq:famo_obj}
\end{equation}
 where $\tilde{\boldsymbol{u}}= (\tilde{u}_1,\dots,\tilde{u}_K )$, $\tilde{u}_k$ is short for $\tilde{u}_k(\boldsymbol{\theta})$.
 % 
 The change of min and max holds due to the linearity of inner term.
 % 
The optimal updating direction reaches at $(\nabla\log \tilde{\boldsymbol{u}})\boldsymbol{p}^* =\boldsymbol{d}^*$.




% a multi-objective optimization, and resolve it with a balanced solution.
% 
To further make the multi-objective optimization, i.e., Eq.~\eqref{eq:famo_obj}, more scalable and adaptive in \problem, we devise an efficient algorithm that reduces the computation and storage burden.
% 
Firstly, we convert the primal problem to its strong dual form, reducing the feasible set.
% 
Then we avoid matrix computation by approximating the gradient based on chain rule. 
% 
In detail, we obtain strong dual form of Eq.~\eqref{eq:famo_obj} that reduces the computation overhead with dual variable $\boldsymbol{p}$:
\begin{equation}
\boldsymbol{J} =\min _{\boldsymbol{p}\in \mathbb{S}^K} \frac{1}{2} \|{(\nabla\log \tilde{\boldsymbol{u}}^t)}\top \boldsymbol{p}\|^2.
\label{eq:famo_dual}
\end{equation}
% 
Then we can substitute iterative optimization for a single-step gradient descent, i.e., $\boldsymbol{\theta}^{t+1} = \boldsymbol{\theta}^t -\eta\nabla\log(\tilde{\boldsymbol{u}})\boldsymbol{p}$.
% 
However, optimizing $\boldsymbol{p}$ is uncontrollable with the constraints of satisfying $\mathbb{S}^K$.
% 
To tackle it, \moduleB~re-parameterizes $\boldsymbol{p}$ by unconstrained logits $\boldsymbol{w}$, i.e., $\boldsymbol{p} = \operatorname{Softmax}(\boldsymbol{w})$,
and optimize via chain rule:
\begin{equation}
\small
\boldsymbol{w}^{t+1} \leftarrow \boldsymbol{w}^t-\beta \left(\nabla_{\boldsymbol{p}} \boldsymbol{J} \nabla_{\boldsymbol{w}} \boldsymbol{p}(\boldsymbol{w})\right),
\end{equation}
where $\beta$ is the step size for logits $\boldsymbol{w}$.
% where $\delta=\nabla_{z} \boldsymbol{J} \nabla_{w} z(\boldsymbol{w})
% =\left(\nabla^{\top} z^1(\boldsymbol{w}), \dots, \nabla^{\top} z^K(\boldsymbol{w})\right)\left(\log \tilde{\boldsymbol{u}}^t-\log \tilde{\boldsymbol{u}}^{t+1}\right)$,
% With global updating $\boldsymbol{\theta}^{t+1} = \boldsymbol{\theta}^t -\eta\nabla\log(\tilde{\boldsymbol{u}})\boldsymbol{p}$,
% 
We then approximate gradient via $\nabla_{\boldsymbol{p}} \boldsymbol{J}= \left(\nabla \log \tilde{\boldsymbol{u}}^t\right)^{\top}\left(\nabla \log \tilde{\boldsymbol{u}}^t\right) \boldsymbol{p}^t \approx \frac{1}{\eta}\left(\log \tilde{\boldsymbol{u}}^t-\log \tilde{\boldsymbol{u}}^{t+1}\right)$, for avoiding the matrix multiplication.
% 
The choice of $\boldsymbol{p}$ simply relies on computing the logarithm of client contribution change in a single step, thus the overall computation and memory cost is scalable for \problem~methods.
% 


Regarding your question, to solve the optimization problem $\boldsymbol{J} =\min _{\boldsymbol{p}} \frac{\eta^2}{2\phi} \|{(\nabla\log \tilde{\boldsymbol{u}})}\top \boldsymbol{p}\|^2 + \lambda \boldsymbol{p}^\top \boldsymbol{1}$ with ADMM, we need to first reformulate the problem into an equivalent form that can be solved using ADMM. 

One way to do this is to introduce an auxiliary variable $\boldsymbol{q}$ and rewrite the problem as follows:

$\boldsymbol{J} =\min _{\boldsymbol{p}, \boldsymbol{q}} \frac{\eta^2}{2\phi} \|{(\nabla\log \tilde{\boldsymbol{u}})}\top \boldsymbol{p}\|^2 + \lambda \boldsymbol{p}^\top \boldsymbol{1} + \frac{\rho}{2} \|\boldsymbol{p} - \boldsymbol{q} + \boldsymbol{z}\|^2$

where $\rho$ is a penalty parameter and $\boldsymbol{z}$ is a Lagrange multiplier. 

Next, we can apply the ADMM algorithm to solve this problem. The ADMM algorithm involves the following steps:

1. Initialize $\boldsymbol{p}$, $\boldsymbol{q}$, and $\boldsymbol{z}$.
2. Repeat until convergence:
   - Update $\boldsymbol{p}$ by minimizing the augmented Lagrangian with respect to $\boldsymbol{p}$:
   
     $\boldsymbol{p}^{k+1} = \arg\min_{\boldsymbol{p}} \frac{\eta^2}{2\phi} \|{(\nabla\log \tilde{\boldsymbol{u}})}\top \boldsymbol{p}\|^2 + \lambda \boldsymbol{p}^\top \boldsymbol{1} + \frac{\rho}{2} \|\boldsymbol{p} - \boldsymbol{q}^{k} + \boldsymbol{z}^{k}\|^2$
     
   - Update $\boldsymbol{q}$ by minimizing the augmented Lagrangian with respect to $\boldsymbol{q}$:
   
     $\boldsymbol{q}^{k+1} = \arg\min_{\boldsymbol{q}}$

how to solve this problem, i.e., $\boldsymbol{J} =\min _{\boldsymbol{p}} \frac{\eta^2}{2\phi} \|{(\nabla\log \tilde{\boldsymbol{u}})}\top \boldsymbol{p}\|^2 + \lambda \boldsymbol{p}^\top \boldsymbol{1}$ with ADMM


\begin{equation}
\small
c_k \left(\eta, \boldsymbol{d}^t\right)=\frac{u_k\left(\boldsymbol{\theta}^{t}_g\right)-u_k\left(\boldsymbol{\theta}^{t+1}_g\right)}{\tilde{u}_k \left(\boldsymbol{\theta}^{t}_g\right)}=\frac{u_k\left(\boldsymbol{\theta}^{t}_g\right)-u_k\left(\boldsymbol{\theta}^{t}_g-\eta \boldsymbol{d}^t\right)}{\tilde{u}_k \left(\boldsymbol{\theta}^{t}_g\right)}, 
\end{equation}
where $\tilde{u}_k\left(\boldsymbol{\theta}^{t}_g\right) = u_k \left(\boldsymbol{\theta}^{t}_g\right)+\epsilon$ is set to prevent zero numerator via adding a minimum $\epsilon$. 
% 
\begin{equation}
\small
\begin{aligned}
c_k \left(\eta, \boldsymbol{d}^t\right)&=\frac{u_k\left(\boldsymbol{\theta}^{t}_g\right)-u_k\left(\boldsymbol{\theta}^{t+1}_g\right)}{\tilde{u}_k \left(\boldsymbol{\theta}^{t}_g\right)}\\
&=\frac{u_k\left(\boldsymbol{\theta}^{t}_g\right)-u_k\left(\boldsymbol{\theta}^{t}_g-\eta \boldsymbol{d}^t\right)}{\tilde{u}_k \left(\boldsymbol{\theta}^{t}_g\right)}\\
&\approx \eta \frac{\nabla \tilde{u}_k(\boldsymbol{\theta}^t) \boldsymbol{d}^t}{\tilde{u}_k(\boldsymbol{\theta})}\\
&= \eta \nabla \log \tilde{u}_k(\boldsymbol{\theta}^t) \boldsymbol{d}^t
\end{aligned}
\end{equation}


% entangles representation collapse because clients model unlabeled data in inconsistent representation spaces.


% Though representation collaspse is widely studied in centralized self-supervised space using (1) contrastive learning, (2) asymmetric architecture modeling~\cite{byol}, and (3) feature decorrelation~\cite{btloss}. 
% % 
% Directly pretraining unlabeled data via existing centralized self-supervised learning, prevents its capability to generalize unified representations.
% % 
% Because these methods
% % Because these methods typically are either explicit or implicit k-Means that suffer from degeneration solutions~\cite{pretrain_longtail}. 


The first challenge is that representation collapse~\cite{collapse_decorr} in the client subsequently exacerbates
 the representation of global and other local models. 
% 
% Existing \problem~methods overlook the representation collapse in modeling real-world applications, where client data follows class-imbalanced, even long-tailed distribution~\cite{imbalancedssl}.
% 
% Some centralized self-supervised learning prevents representation collapse via measuring covariance rank~\cite{simclr_collapse,simsiam_collapse}.
% for contrastive based methods~\cite{simclr_collapse}, and non-contrastive based methods~\cite{simsiam_collapse}.
% 
% But these methods typically are either explicit or implicit k-Means for balanced datasets~\cite{pretrain_longtail}, which suffer from degeneration solutions when data is non-IID. 
% It is limited to directly apply for \problem, especially cross-device setup, since it relies on large batch size~\cite{orchestra} to capture reliable representation variance.\xenia{confirm}
% 
% In federated supervised learning, FedDecorr~\cite{feddecorr} analyzes the dimensional collapse of global model via gradient dynamics of cross-entropy loss.
% 
Motivated by regularizing Frobenius norm of representation in centralized self-supervised models~\cite{simclr_collapse,simsiam_collapse}, FedDecorr~\cite{feddecorr} tackles representation collapse with the global supervision signals in federated supervised learning.
% finds that the dimensional collapse in client model will subsequently deteriorate the representation of global and other local models in an entangled way. 
%
% 
But directly applying these methods to \problem~has three aspects of limitations.
% 
Firstly, it relies on large data batch size~\cite{orchestra} to capture reliable distribution statistics, e.g., representation variance.
% 
Besides, regularizing the norm of high-dimensional representations inevitably causes inactivated neurons and suppresses meaningful features~\cite{featuresupress}.
% 
Lastly, lacking unified representation spaces, each client fails to decorrelate representation consistently, unsolving representation collapse entanglement.





Multi-objective optimization is promising to resolve the inconsistencies and conflicts among clients~\cite{fedmgda+}.
% 
Motivated by this, we decide to re-organize the aggregation, i.e., Eq.~\eqref{eq:fusl_problem} as a multi-task of optimizing the client contribution rate, i.e., the local-global model deviation change rate between two communication rounds.
% 
% 
Based on the measure of contribution rate, there are two goals of \moduleB, i.e., (1) maximizing the global updating direction $\boldsymbol{d}^t$ away from the worst overall contribution rate, and (2) making the contribution rate for $k \in [K]$ as balanced as possible to obtain consistent model parameters.
% 


To reach the first goal, we define the client contribution rate in the following.
%
In round $t$, let global model before aggregation as $\boldsymbol{\theta}_g^{t}$, and global model after aggregation as $\boldsymbol{\theta}_g^{t+1}=\boldsymbol{\theta}_g^{t} - \eta \boldsymbol{d}^t$ which updates toward direction $\boldsymbol{d}^t$ with step size $\eta$.
% 
\moduleB~measures the \xenia{model deviation} of $k$-th client model $\boldsymbol{\theta}_k^t$, i.e., $u_k(\boldsymbol{\theta}^{t}_g)=\| \boldsymbol{\theta}^{t}_g - \boldsymbol{\theta}^{t}_k\|^2$ and $u_k^t$ for short.\xenia{define deviation}
% and $u_k(\boldsymbol{\theta}^{t+1}_g, \boldsymbol{\theta}^t_k)=\| \boldsymbol{\theta}^{t+1}_g - \boldsymbol{\theta}^t_k\|^2$ for global model before and after aggregation, respectively.
% 
Assuming step size $\eta$ is small,
the contribution change can be approximated as $\Delta {u_k^t} =u_k\left(\boldsymbol{\theta}^{t}_g\right)-u_k\left(\boldsymbol{\theta}^{t+1}_g\right) \approx \eta \nabla \tilde{u}_k(\boldsymbol{\theta}^{t}_g)\boldsymbol{d}^t$.
% 
Then the contribution rate of client $k$ is:
\begin{equation}
\small
\begin{aligned}
c_k \left(\eta, \boldsymbol{d}^t\right)=\frac{u_k\left(\boldsymbol{\theta}^{t}_g\right)-u_k\left(\boldsymbol{\theta}^{t+1}_g\right)}{\tilde{u}_k \left(\boldsymbol{\theta}^{t}_g\right)}
\approx \eta \nabla \log \tilde{u}_k(\boldsymbol{\theta}^t_g) \boldsymbol{d}^t
\end{aligned}
\end{equation}
where $\tilde{u}_k\left(\boldsymbol{\theta}^{t}_g\right) = u_k \left(\boldsymbol{\theta}^{t}_g\right)+\epsilon$ is set to prevent zero numerator via adding a minimum $\epsilon>0$.\xenia{del}
% 
The client contribution rate $c_k \left(\eta, \boldsymbol{d}^t\right)$ captures the model deviation from client $k$ to global model between two communication rounds, indicating the impact of client $k$ in global aggregation.
% % 
For example, in \moduleB~of Fig.~\ref{fig:model}, the contribution rate of client 1 is larger than client 2, i.e., $c_1 \left(\eta, \boldsymbol{d}^t\right)> c_2 \left(\eta, \boldsymbol{d}^t\right)$, making the model in client 1 to approaches global optimum, while the model in client 2 deviates.


With reference to client contribution rate, we further define the multi-objective optimization which seeks a direction maximizing the worst overall client contribution rate:
\begin{equation}
\small
\begin{aligned}
\max _{\boldsymbol{d}^t \in \mathbb{R}^{K\times m}} \min _{\boldsymbol{p} \in \mathbb{S}^K} {\eta} \sum_{k=1}^{K} p_k \nabla \log \tilde{u}_k(\boldsymbol{\theta}^t_g) \boldsymbol{d}^t,\\
s.t. \|\boldsymbol{d}^t\|^2 \leq 1, \boldsymbol{p}^\top \boldsymbol{1} =1 .
\end{aligned}
\label{eq:mtl_cc}
\end{equation}
% and $\mathbb{S}^K=\{\boldsymbol{p}\in \mathbb{R}^K | \boldsymbol{p}^\top \boldsymbol{1}=1\}$.
% 
